Variational Inverse Control with Events: A General Framework for Data-Driven Reward Definition

The design of a reward function often poses a major practical challenge to real-world applications of reinforcement learning. Approaches such as inverse reinforcement learning attempt to overcome this challenge, but require expert demonstrations, which can be difficult or expensive to obtain in practice. We propose variational inverse control with events (VICE), which generalizes inverse reinforcement learning methods to cases where full demonstrations are not needed, such as when only samples of desired goal states are available. Our method is grounded in an alternative perspective on control and reinforcement learning, where an agent's goal is to maximize the probability that one or more events will happen at some point in the future, rather than maximizing cumulative rewards. We demonstrate the effectiveness of our methods on continuous control tasks, with a focus on high-dimensional observations like images where rewards are hard or even impossible to specify.

==> paper/4_variational.tex <==
\section{Control as Variational Inference}
\label{sec:variational_inf}
%
Performing inference directly in the graphical model in Figure~\ref{fig:controlgraph} produces solutions that are optimistic with respect to stochastic dynamics, and produces risk-seeking behavior. This is because posterior inference is not constrained to force $p(s_{t+1}|s_t,a_t,e_{1:T}) = p(s_{t+1}|s_t,a_t)$: that is, it assumes that, like the action distribution, the next state distribution will ``conspire'' to make positive outcomes more likely. Prior work has sought to address this issue via the framework of causal entropy~\citep{Ziebart10}. To provide a more unified treatment of control as inference, we instead present a variational inference derivation that also addresses this problem. We will use this method to derive new policy objectives in Section~\ref{sec:event_based_control}, while in this section we derive it in the context of standard maximum entropy reinforcement learning.

When conditioning the graphical model in Figure~\ref{fig:controlgraph} on $e_{1:T}=1$ as before, the optimal trajectory distribution is
\[
p(\tau|e_{1:T}) \propto p(s_1)\prod_{t=1}^{T-1} p(s_{t+1}|s_t,a_t)p(a_t|s_t)e^{r(s,a)}.
\]
We will assume that the action prior $p(a_t|s_t)$ is uniform without loss of generality, since non-uniform distributions can be absorbed into the reward term $e^{r(s,a)}$, as discussed in Appendix~\ref{app:event_derivations_mprl}.

The correct maximum entropy reinforcement learning objective emerges when performing variational inference in this model, with a variational distribution of the form \mbox{$q_\theta(\tau) = p(s_1)\prod_{t=1}^{T-1} p(s_{t+1}|s_t,a_t)q_\theta(a_t|s_t)$}. In this distribution, the initial state distribution and dynamics are forced to be equal to the true dynamics, and only the action conditional $q_\theta(a_t|s_t)$, which corresponds to the policy, is allowed to vary. Writing out the variational objective and simplifying, we get
\begin{align*}
-D_{KL}(q_\theta(\tau) || &p(\tau|e_{1:T}))
=
E_{\tau \sim q(\tau)}\left[\sum_{t=1}^T r(s_t,a_t) - \log q_\theta(a|s) \right].
\end{align*}
We see that we obtain the same problem as (undiscounted) entropy-regularized reinforcement learning, where $q_\theta(a|s)$ serves as the policy. For more in-depth discussion, see Appendix~\ref{app:event_derivations_causal_all}. We can recover the discounted objective by modifying the dynamics such that the agent has a $(1-\gamma)$ probability of transitioning into an absorbing state with 0 reward. 

We have thus derived how maximum entropy reinforcement learning can be recovered by applying variational inference with a specific choice of variational distribution to the graphical model in Figure~\ref{fig:controlgraph}. In the next section, we will extend this method to get rid of the arbitrary reward function and replace it with a more interpretable notion of events.


==> paper/acknowledgements.tex <==
\section*{Acknowledgements}

\textbf{Do not} include acknowledgements in the initial version of
the paper submitted for blind review.

If a paper is accepted, the final camera-ready version can (and
probably should) include acknowledgements. In this case, please
place such acknowledgements in an unnumbered section at the
end of the paper. Typically, this will include thanks to reviewers
who gave useful comments, to colleagues who contributed to the ideas,
and to funding agencies and corporate sponsors that provided financial
support.


==> paper/multiobjective.tex <==
%
%

%

%

%
%
%
%
%
%
%
%
%


==> paper/rewards_to_events.tex <==
\section{From Rewards to Events}
\label{sec:events}

We previously chose \mbox{$\log p(e_t=1|s_t,a_t) = r(s,a)$} so that the objective of the resulting inference problem matches the maximum entropy reinforcement learning objective. However, we might also ask: what does the variable $e_t$, and its probability, actually represent in this case? The connection to graphical models gives us a potential answer: rewards represent the log-probability that a desired event happens given some state and action of the agent, and the standard approach to reward engineering can also be viewed as designing the probability of some binary event, that we might call an optimality event. %
This provides us with a convenient way to think about reward design: instead of designing arbitrary scalar fields, what if we directly specify the events for which we would like to maximize the probability of occurrence?

\begin{figure}[tb]
\centering
\includegraphics[width=0.7\columnwidth]{img/trashbug_env}
\caption{
\label{fig:trashbug}
The gold miner toy domain. The agent starts in the upper left with a low quality mine, with a small chance of finding real gold and high chance of finding fool's gold. In the bottom right there is a high quality mine that always produces real gold. The agent can move up, down, left, right, or do nothing. Black tiles represent walls.
}
\end{figure}

For an example where rethinking rewards as events can change how we design control problems, consider the toy gridworld domain shown in Figure~\ref{fig:trashbug}. We have a simple delayed reward example where the miner must choose between mining in a nearby but low-yield mine and a far away but high-yield mine. In the low-yield mine, the miner has a small chance of finding real gold and a high chance of finding fool's gold. In the high-yield mine, the miner is guaranteed to find real gold. The miner cannot tell the difference between real gold and fool's gold. This situation is quite realistic in practical RL problems, where there can be considerable uncertainty about whether a task has been successfully achieved. For example, a household robot may need to guess whether it has cleaned the house properly as commanded by its owner, and a technical support chatbot might be able to get only an indirect measure of customer satisfaction based on sentiment analysis.
%

In a standard reinforcement learning scenario, we may choose to place a large reward, say $+10$, on the states that are more likely to produce a success, which in this case is the high-yield mine, and a small reward, such as $+1$, on the low-yield mine. Depending on the dynamics and discount factor, the miner may choose to stay at the low-yield mine or move to the high-yield mine. Reasoning about what values to choose for rewards is difficult to reason about, in part because of the intricate dependency to the dynamics of the model, distance to reward sites, and discout factor.
%

In the event-based framework, we think in terms of probabilities of events. So we would say that, at the low-yield mine, there is a $10\%$ chance of finding gold, and at the high-yield mine there is a $100\%$ chance. Everywhere else, the chance is $0\%$. We can now select for different behavior depending on which inference problem we pose for the graphical model. If we would like to maximize the probability that the miner will find gold at every single time step, the optimal behavior is to remain at the low-yield mines. Under this strategy, there is a positive probability that the miner will never receive gold, but there is a chance that he will receive gold at all time steps. However, if instead we ask for gold to be found on at least one time step, then the agent will instead seek out the high-yield mine, since it results in at least one guaranteed success, even though many time steps will contain no success. The desired behavior can be clearly captured by performing inference with the right type of evidence, without further tuning of the problem statement.

%
%
%
